A Call for Critically Rethinking and Reforming Data Analysis in Empirical Software Engineering

Context: Empirical Software Engineering (ESE) drives innovation in SE through qualitative and quantitative studies. However, concerns about the correct application of empirical methodologies have existed since the 2006 Dagstuhl seminar on SE. Objective: To analyze three decades of SE research, identify mistakes in statistical methods, and evaluate experts' ability to detect and address these issues. Methods: We conducted a literature survey of ~27,000 empirical studies, using LLMs to classify statistical methodologies as adequate or inadequate. Additionally, we selected 30 primary studies and held a workshop with 33 ESE experts to assess their ability to identify and resolve statistical issues. Results: Significant statistical issues were found in the primary studies, and experts showed limited ability to detect and correct these methodological problems, raising concerns about the broader ESE community's proficiency in this area. Conclusions. Despite our study's eventual limitations, its results shed light on recurring issues from promoting information copy-and-paste from past authors' works and the continuous publication of inadequate approaches that promote dubious results and jeopardize the spread of the correct statistical strategies among researchers. Besides, it justifies further investigation into empirical rigor in software engineering to expose these recurring issues and establish a framework for reassessing our field's foundation of statistical methodology application. Therefore, this work calls for critically rethinking and reforming data analysis in empirical software engineering, paving the way for our work soon.

==> Sections/Discussions.tex <==
This section discusses our findings. This study serves as a pilot for our broader, ongoing evaluation of state-of-the-art literature across all digital libraries, extending beyond the current paper selection and the investigation scope.

The analysis of the publication trends in ESE, i.e. RQ$_2$ gives several interesting insights about the development of methodological practices within the field. The interest of scholars has increased steadily over the years, culminating in a record number of publications in 2023, indicating a living and growing research community. However, taking a closer look at the methodological trends reveals huge gaps. Quantitative studies are dominant in the landscape, which shows a preference for measurable and numeric data, while qualitative studies are notably underrepresented. This may indicate that there is a preference in the subject area for precision and generalizability over exploratory or contextual insights.

The trend realized in the checking of distribution of data is worrying. Very few checked the distribution of their data, and out of them, an even smaller fraction checked normality. Given that many statistical tests are based on the assumption of normal distribution, this step, if ignored, may lead to the failure of the results. Similarly, the trend in hypothesis testing shows that although some studies do this important thing, many do not, and most lean toward simpler analyses of correlation or non-parametric tests. This indicates a limited engagement with robust statistical methods that may reduce the robustness and reliability of conclusions made.

These trends do indeed indicate the need for more rigorous methodological thresholds in ESE research. Such checks on distribution should be comprehensive; encouraging a culture of robust testing of hypotheses will serve to increase the credibility and impact of future studies.

More specifically, RQ$_2$ reveals that over the last 30 years, various methodological issues have impacted the ESE field. In particular, problems such as the blind application of tests without considering their prerequisites, i.e., like testing the distribution and shape of the data, threatens the validity and generalizability of many ESE studies.

%In the same vein, the results from $RQ_2$ indicate unexpected behaviors. 
Finally, according to our findings in RQ$_3$ and RQ$_4$, we showed that the \textbf{experts confounded statistics principles} in reviewing the excerpts from the paper.  According to Figure \ref{fig:synth}, experts often wrongly suggested new statistical tests or different models and techniques. Moreover, our findings further highlight significant flaws in the peer-review process, as experts frequently misidentify appropriate statistical tests, models, and methods. As also highlighted by  Prof. Sira Vegas in the ESEIW 2024 keynote on methodological issues in deep learning studies in ESE \footnote{\url{https://conf.researchr.org/info/esem-2024/keynotes}}. Therefore, considering all these findings and the fact that our study stemmed from our own peer-review experience and the legacy of the 2006 Dagstuhl seminar, we can affirm that the problem exists and is unfortunately widespread all across our community. 



 %A recurring joke around academic social networks regards the different patches and modifications reviewers suggest during the peer-review process. It is a common feeling to modify our manuscripts to provide new statistical test results or model and technique comparisons. 

==> Sections/Results.tex <==
This section presents the early findings from our pilot and the workshop. 

\subsection{Historical Trends in Empirical Data Analysis Methodology (\texorpdfstring{RQ$_1$}{RQ1})}
Figure \ref{fig:pubtrend} shows the ESE publication trend in the selected venues. According to Figure \ref{fig:pubtrend}, since the mid-90s, the interest in our field has kept increasing, reaching the top of more than 800 papers published in a single year (2023). Following this preliminary trend, we are interested in analyzing in depth the trend of the methodological choices in terms of Variable type, data distribution checks, and hypothesis testing.

Figure \ref{fig:vartypetrend} presents the study's variable type trend. According to Figure \ref{fig:vartypetrend}, quantitative studies are consistently the most preferred analyzed variable with a consistent gap from qualitative ones. Conversely, the variable under examination was negligible in mixed and unclear studies.

Furthermore, Figure \ref{fig:distrtrend} presents the study's variable distributional checks trend. According to Figure \ref{fig:distrtrend}, authors rarely check for the distribution of the variables, and among the few that do that, a very handful of them check for normality. Normal distribution is a prerequisite for specific hypothesis testing and analysis methods. Not checking the distribution and applying an erroneous test threaten the entire validity of the study.

Finally, Figure \ref{fig:hypotesttrend} presents the study's hypothesis testing trend. According to Figure \ref{fig:hypotesttrend}, most works do not test the hypothesis. Most studies that test their hypothesis test correlations or use non-parametric or distribution-specific tests.

Therefore, we can observe that over the last decade \textbf{authors focused on quantitative study, rarely checking the distribution of the collected data or testing their hypothesis}.


\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{Figures/Trends/Publication Trend.pdf}
    \caption{Empirical Software Engineering Publication Trend}
    \label{fig:pubtrend}
\end{figure}


\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{Figures/Trends/Var Type Trend.pdf}
    \caption{Variable Type Trend}
    \label{fig:vartypetrend}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{Figures/Trends/Distribution Category.pdf}
    \caption{Distribution Check Trend}
    \label{fig:distrtrend}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{Figures/Trends/Hypothesis Testing.pdf}
    \caption{Hypothesis Testing Trend}
    \label{fig:hypotesttrend}
\end{figure}


\subsection{Common Methodology Patterns in Empirical Data Analysis (\texorpdfstring{RQ$_2$}{RQ2})}

Figure \ref{fig:sanky} presents the Sanky Diagram, highlighting an example of flawed pattern. According to Figure \ref{fig:sanky}, roughly 90\% of papers focusing on Quantitative or Qualitative data did not check the distribution of the collected data. We refer to this set of papers as \textbf{$\mathcal{A}$}. About 10\% of $\mathcal{A}$ proceeded with parametric tests, which require data normally distributed, and 90\% of them did not employ any post hoc correction.

In the same vein, 15\% of \textbf{$\mathcal{A}$} performed a distribution-specific test without being aware of the data distribution.


Therefore, we can observe that \textbf{different methodological issues affect the last 30 years of ESE}.


\subsection{Accuracy of ESE Experts in Detecting Flawed Methodological Patterns (\texorpdfstring{RQ$_3$}{RQ3})}
Figure \ref{fig:summary}  presents the distribution of good and flawed guesses from the experts summarized by the taxonomy category. According to Figure \ref{fig:summary}, the experts did not reliably spot methodological flaws. On the one hand, the experts could not reliably identify the variable types, appropriate models or methods, and post hoc tests needed for the study. This led to misclassification, i.e., labeling poor analyses as good and vice versa. On the other hand, the experts reliably classified the data distribution checks correctly. 
Therefore, we can observe that on average, \textbf{ESE experts show limited precision in accurately reviewing methodologies based on our taxonomy}.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/Summary.pdf}
    \caption{Good and Flawed Methodological Patterns Distribution Guesses from Experts by Category}
    \label{fig:summary}
\end{figure*}

\subsection{ESE Experts’ Accuracy in Recommending Remediations for Flawed Methodological Patterns (\texorpdfstring{RQ$_4$}{RQ4})}

Figure \ref{fig:synth} shows the distribution of flawed and good guesses from the experts by specific answers. According to Figure \ref{fig:synth}, referring to the findings in Figure \ref{fig:summary}, most of the errors the expert committed during the evaluation are in the other suggestions keyword. Hence, in most cases, when the expert suggested a different technique, model, or statistical test, the suggestion itself was wrong.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{Figures/Synthesis.pdf}
    \caption{Distribution of Flawed and Good Guesses from Experts by Answer}
    \label{fig:synth}
\end{figure}


Finally, according to our results on the accuracy metrics computed for the expert across the seven groups and the provided scenarios with the overall evaluation of the papers provided, we note that the experts underperformed in each accuracy metric. 

More specifically, experts scored very low accuracy in terms of Recall (0.3846), Precision (0.3846),  Accuracy (0.3600),  F1-Score (0.3846), and a negative MCC (-0.2821).

Therefore, we can observe that \textbf{experts, on average, were not able to identify statistical methodological issues}.

%\input{Tables/Accuracy}


==> Tables/Accuracy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}
\centering
\small
\caption{Expert's Accuracy Metrics}
\label{tab:accuracy}

\begin{tabular}{lllll}
\hline
Recall & Precision & Accuracy & F1-Score & MCC     \\ \hline
0.3846 & 0.3846    & 0.3600   & 0.3846   & -0.2821 \\ \hline
\end{tabular}
\end{table}
